PCA-Based Knowledge Distillation Towards Lightweight and Content-Style Balanced Photorealistic Style Transfer Models

Photorealistic style transfer entails transferring the style of a reference image to another image so the result seems like a plausible photo. Our work is inspired by the observation that existing models are slow due to their large sizes. We introduce PCA-based knowledge distillation to distill lightweight models and show it is motivated by theory. To our knowledge, this is the first knowledge distillation method for photorealistic style transfer. Our experiments demonstrate its versatility for use with different backbone architectures, VGG and MobileNet, across six image resolutions. Compared to existing models, our top-performing model runs at speeds 5-20x faster using at most 1\% of the parameters. Additionally, our distilled models achieve a better balance between stylization strength and content preservation than existing models. To support reproducing our method and models, we share the code at \textit{https://github.com/chiutaiyin/PCA-Knowledge-Distillation}.

==> backup.tex <==
\subsection{Preliminaries: Neural Style Transfer}
\label{sec:reformulated_nst}
Neural Style Transfer (NST), the seminal work of applying a neural network to artistic style transfer, represents the content of an image with its feature $\mathbf{F}_N$ $\in$ $C_N\times H_NW_N$\footnote{$\mathbf{F}_N$ is a 3D tensor $\in$ $C_N\times H_N\times W_N$ when output from a VGG layer. For convenience, we treat it as a 2D matrix in the paper. } extracted at an intermediate $\textit{reluN\_1}$ layer of VGG-19, and the style of the image with the Gram matrix $\frac{1}{H_NW_N}\mathbf{F}_N\mathbf{F}^\mathrm{T}_N$. Usually, a later layer (e.g. $\textit{relu4\_1}$) of VGG-19 is adopted for the content representation extraction, since it captures the high-level content information but discards the detailed pixel values/color of the image. To capture both global and local textures of the image, multiple layers (e.g. $\textit{reluN\_1}$, $N$ $=$ $1,2,3,4$) are used for style representation extraction. 

Let $\mathbf{F}_{N,x}$ denote the feature of the image $I_x$ extracted at the $\textit{reluN\_1}$ layer. Given a content image $I_c$ and a style image $I_s$, NST is searching a stylized image $I_{t}$ whose content representation is close to that of $I_c$ and style representation is close to that of $I_s$. Mathematically, it solves the following optimization problem by back-propagation.
\begin{equation}
\small
    \min_{I_{t}} ||\mathbf{F}_{4,c}-\mathbf{F}_{4,t}||_2^2 + \lambda \sum_{N=1}^4 ||\text{Gram}(\mathbf{F}_{N,s}) - \text{Gram}(\mathbf{F}_{N,t})||^2_2,
    \label{eq:nst}
\end{equation}
where $\lambda$ controls the style transfer strength. \cref{eq:nst_cov} and \cref{eq:nst_cov_fbar} are two variations of \cref{eq:nst}:
\begin{equation}
\small
    \min_{I_{t}} ||\mathbf{F}_{4,c}-\mathbf{F}_{4,t}||_2^2 + \lambda \sum_{N=1}^4 ||\text{Cov}(\mathbf{F}_{N,s}) - \text{Cov}(\mathbf{F}_{N,t})||^2_2,
    \label{eq:nst_cov}
\end{equation}
where the style representation is the covariance of a feature $\mathbf{F}_{N}$ equal to $\frac{1}{H_NW_N}\mathbf{\bar{F}}_{N}\mathbf{\bar{F}}_{N}^\mathrm{T}$ with $\mathbf{\bar{F}}_{N}$ being the centralized feature $\mathbf{F}_{N}-\mu(\mathbf{F}_{N})$, where $\mu(\mathbf{F}_N)$ is the mean of $H_NW_N$ column vectors of $\mathbf{F}_N$, and
\begin{equation}
\small
    \min_{I_{t}} ||\mathbf{\bar{F}}_{4,c}-\mathbf{\bar{F}}_{4,t}||_2^2 + \lambda \sum_{N=1}^4 ||\text{Cov}(\mathbf{F}_{N,s}) - \text{Cov}(\mathbf{F}_{N,t})||^2_2,
    \label{eq:nst_cov_fbar}
\end{equation}
where the centralized feature $\mathbf{\bar{F}}_N$ is used as the content representation. 



The third column of \cref{fig:reformulated_nst} shows two examples of stylized images using the NST algorithm.

However, we hardly extend from the Gram matrix representation to develop an algorithm to distill the essential style knowledge from VGG-19 and meanwhile avoid the nonessential that causes artifacts in order for better photorealism. Therefore, we consider to use the covariance matrix $\frac{1}{H_NW_N}\mathbf{\bar{F}}_N\mathbf{\bar{F}}^\mathrm{T}_N$ for the style representation\footnote{\color{red} Much of the literature which cites the NST paper misuses the terms Gram matrix and covariance matrix interchangeably due to their similar forms. However, they are two fundamentally different statistics and NST uses Gram matrices but not covariance matrices.}, where $\mathbf{\bar{F}}_N$ is the centralized feature of $\mathbf{F}_N$ defined as
\begin{equation}
    \mathbf{\bar{F}}_N = \mathbf{F}_N - \mu(\mathbf{F}_N) = \mathbf{F}_N - \frac{1}{HW}\sum_{i=1}^{HW} \mathbf{F}_{N[:,i]},
\end{equation}
where $\mu(\mathbf{F}_N)$ is the mean of $HW$ column vectors of $\mathbf{F}_N$. Since the covariance matrix of data points is related to their principle components, which can be exploited for dimension reduction with the essential information preserved, we can anticipate a knowledge distillation for photorealistic style transfer if the covariance matrix is a valid style representation.

Note that different from the closest prior work of WCT, which matches both the mean $\mu(\mathbf{F}_{N,t})$ and the covariance matrix $\frac{1}{H_{N,t}W_{N,t}}\mathbf{\bar{F}}_{N,t}\mathbf{\bar{F}}^\mathrm{T}_{N,t}$ of the stylized image $I_t$ to those ($\mu(\mathbf{F}_{N,s})$ and $\frac{1}{H_{N,s}W_{N,s}}\mathbf{\bar{F}}_{N,s}\mathbf{\bar{F}}^\mathrm{T}_{N,s}$) of the style image $I_s$, we exclude the effect of mean and consider the covariance matrix as the \textbf{only} influencing factor. In fact, WCT still falls in the regime of Gram matrix matching, since matching to the mean and covariance matrix is a special case of matching to the Gram matrix:
\begin{equation}
    \begin{aligned}
    &\frac{1}{n_t}\mathbf{F}_{N,t}\mathbf{F}^\mathrm{T}_{N,t} 
    = \frac{1}{n_t}\mathbf{\bar{F}}_{N,t}\mathbf{\bar{F}}^\mathrm{T}_{N,t} + \mu(\mathbf{F}_{N,t})\mu(\mathbf{F}_{N,t})^\mathrm{T} \\
    = &\frac{1}{n_s}\mathbf{\bar{F}}_{N,s}\mathbf{\bar{F}}^\mathrm{T}_{N,s} + \mu(\mathbf{F}_{N,s})\mu(\mathbf{F}_{N,s})^\mathrm{T} 
    = \frac{1}{n_s}\mathbf{F}_{N,s}\mathbf{F}^\mathrm{T}_{N,s},
    \end{aligned}
\end{equation}
where $n_t$ $=$ $H_{N,t}W_{N,t}$ and $n_s$ $=$ $H_{N,s}W_{N,s}$.

To test if a covariance matrix can be a style representation, we replace the Gram matrices in \cref{eq:nst} with the covariance matrices and solve the following reformulated optimization problem.
\begin{equation}
    \min_{I_{t}} ||\mathbf{F}_{4,c}-\mathbf{F}_{4,t}||_2^2 + \lambda \sum_{N=1}^4 ||\text{Cov}(\mathbf{F}_{N,s}) - \text{Cov}(\mathbf{F}_{N,t})||^2_2.
    \label{eq:reformulated_nst}
\end{equation}
The fourth column of \cref{fig:reformulated_nst} shows two stylized results from \cref{eq:reformulated_nst}. We observe that by matching covariance matrices the style can also be transferred to the content image. Moreover, we notice that the same style can manifest differently between Gram matrix matching and covariance matrix matching. These observations imply that the covariance matrix is a legit style representation.

For the consistency with the use of the centralized feature $\mathbf{\bar{F}}_N$ in the covariance style representation $\frac{1}{H_NW_N}\mathbf{\bar{F}}_N\mathbf{\bar{F}}^\mathrm{T}_N$, we also study the use of $\mathbf{\bar{F}}_N$ as the content representation: we replace the first term in \cref{eq:reformulated_nst} with $||\mathbf{\bar{F}}_{4,c}-\mathbf{\bar{F}}_{4,t}||_2^2$ and solve the optimization problem. The fourth and fifth columns of \cref{fig:reformulated_nst} show that $\mathbf{\bar{F}}_N$ as the content representation has a similar effect to $\mathbf{F}_N$ when coupled with the covariance style representation and so is a valid representation. In Experiments, we use $\mathbf{\bar{F}}_N$ and $\frac{1}{H_NW_N}\mathbf{\bar{F}}_N\mathbf{\bar{F}}^\mathrm{T}_N$ as metrics to evaluate the content-style balance.



%%%%%

Mathematically, it solves the following optimization problem by back-propagation.
\begin{equation}
\small
    \min_{I_{t}} ||\mathbf{F}_{4,c}-\mathbf{F}_{4,t}||_2^2 + \lambda \sum_{N=1}^4 ||\text{Gram}(\mathbf{F}_{N,s}) - \text{Gram}(\mathbf{F}_{N,t})||^2_2,
    \label{eq:nst}
\end{equation}
where $\lambda$ controls the style transfer strength. We further consider two variations of \cref{eq:nst} in \cref{eq:nst_cov} and \cref{eq:nst_cov_fbar}:
\begin{equation}
\small
    \min_{I_{t}} ||\mathbf{F}_{4,c}-\mathbf{F}_{4,t}||_2^2 + \lambda \sum_{N=1}^4 ||\text{Cov}(\mathbf{F}_{N,s}) - \text{Cov}(\mathbf{F}_{N,t})||^2_2,
    \label{eq:nst_cov}
\end{equation}
where we test if the covariance of a feature $\mathbf{F}_{N}$ is a valid style representation and $\text{Cov}(\mathbf{F}_{N})$ equals to $\frac{1}{H_NW_N}\mathbf{\bar{F}}_{N}\mathbf{\bar{F}}_{N}^\mathrm{T}$ with $\mathbf{\bar{F}}_{N}$ being the centralized feature $\mathbf{F}_{N}-\mu(\mathbf{F}_{N})$, where $\mu(\mathbf{F}_N)$ is the mean of $H_NW_N$ column vectors of $\mathbf{F}_N$. 

Since NST consistently use the uncentralized feature in both content and style representations, to be consistent with the centralized feature $\mathbf{\bar{F}}_N$ in the covariance style representation in \cref{eq:nst_cov}, we also test if $\mathbf{\bar{F}}_N$ as the content representation affects the validity of covariance style representation:
\begin{equation}
\small
    \min_{I_{t}} ||\mathbf{\bar{F}}_{4,c}-\mathbf{\bar{F}}_{4,t}||_2^2 + \lambda \sum_{N=1}^4 ||\text{Cov}(\mathbf{F}_{N,s}) - \text{Cov}(\mathbf{F}_{N,t})||^2_2.
    \label{eq:nst_cov_fbar}
\end{equation}
The \cref{fig:reformulated_nst} shows that matching $\text{Cov}(\mathbf{F}_{N,t})$ to $\text{Cov}(\mathbf{F}_{N,s})$ not only transfers the style of $I_s$ to $I_t$ but makes the style manifest differently from the Gram matrix matching, implying the covariance is a legit style representation. We also notice whether the content feature is centralized for the content representation does not affect the validity of the covariance style representation.

Note that different from the closest prior work of WCT, which matches both the mean $\mu(\mathbf{F}_{N,t})$ and the covariance matrix $\frac{1}{H_{N,t}W_{N,t}}\mathbf{\bar{F}}_{N,t}\mathbf{\bar{F}}^\mathrm{T}_{N,t}$ of the stylized image $I_t$ to those ($\mu(\mathbf{F}_{N,s})$ and $\frac{1}{H_{N,s}W_{N,s}}\mathbf{\bar{F}}_{N,s}\mathbf{\bar{F}}^\mathrm{T}_{N,s}$) of the style image $I_s$, we exclude the effect of mean and consider the covariance matrix as the \textbf{only} influencing factor. In fact, WCT still falls in the regime of Gram matrix matching, since matching to the mean and covariance matrix is a special case of matching to the Gram matrix:
\begin{equation}
\small
    \begin{aligned}
    &\frac{1}{n_t}\mathbf{F}_{N,t}\mathbf{F}^\mathrm{T}_{N,t} 
    = \frac{1}{n_t}\mathbf{\bar{F}}_{N,t}\mathbf{\bar{F}}^\mathrm{T}_{N,t} + \mu(\mathbf{F}_{N,t})\mu(\mathbf{F}_{N,t})^\mathrm{T} \\
    = &\frac{1}{n_s}\mathbf{\bar{F}}_{N,s}\mathbf{\bar{F}}^\mathrm{T}_{N,s} + \mu(\mathbf{F}_{N,s})\mu(\mathbf{F}_{N,s})^\mathrm{T} 
    = \frac{1}{n_s}\mathbf{F}_{N,s}\mathbf{F}^\mathrm{T}_{N,s},
    \end{aligned}
\end{equation}
where $n_t$ $=$ $H_{N,t}W_{N,t}$ and $n_s$ $=$ $H_{N,s}W_{N,s}$.



\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/reformulated_NST.jpg}
    \caption{Neural Style Transfer (NST) and two variants. NST (col 3) uses the uncentralized feature $\mathbf{F}$ as the content representation (CR) and the Gram matrix $\mathbf{F}\mathbf{F}^\mathrm{T}$ as the style representation (SR), while the variants use the covariance matrix $\mathbf{\bar{F}}\mathbf{\bar{F}}^\mathrm{T}$ as the SR and the uncentralized feature $\mathbf{F}$ (col 4) or the centralized feature $\mathbf{\bar{F}}$ (col 5) as the CR. The results show that using the covariance matrix as the SR presents the style differently than the gram matrix (several differences are emphasized with colored boxes) and whether the CR is centralized does not affect much.}
    \vspace{-2mm}
    \label{fig:reformulated_nst}
\end{figure}

The \cref{fig:reformulated_nst} shows that matching $\text{Cov}(\mathbf{F}_{N,t})$ to $\text{Cov}(\mathbf{F}_{N,s})$ makes the style manifest differently from the Gram matrix matching, and whether the content feature is centralized for the content representation does not affect much.
